IntactKV: Improving Large Language Model Quantization by Keeping Pivot Tokens Intact

Large language models (LLMs) excel in natural language processing but demand intensive computation. To mitigate this, various quantization methods have been explored, yet they compromise LLM performance. This paper unveils a previously overlooked type of outliers in LLMs. Such outliers are found to allocate most of the attention scores on initial tokens of input, termed as pivot tokens, which are crucial to the performance of quantized LLMs. Given that, we propose IntactKV to generate the KV cache of pivot tokens losslessly from the full-precision model. The approach is simple and easy to combine with existing quantization solutions with no extra inference overhead. Besides, IntactKV can be calibrated as additional LLM parameters to boost the quantized LLMs further with minimal training costs. Mathematical analysis also proves that IntactKV effectively reduces the upper bound of quantization error. Empirical results show that IntactKV brings consistent improvement over various quantization methods across different LLMs and downstream tasks, leading to the new state-of-the-art for LLM quantization. The codes are available at https://github.com/ruikangliu/IntactKV.

==> latex/texes/acknowledge.tex <==
\section*{Acknowledgements}

==> latex/texes/table_back.tex <==

\paragraph{Results on MMLU tasks.}
\lin{Need to rewrite.}
We first implement our PRONG approach on INT3-g128 quantized Vicuna models with AWQ method.
Table \ref{tab:mmlu} presents the zero-shot and five-shot results on MMLU benchmarks across varying model sizes.
In the five-shot evaluation, PRONG leverages the full-precision Key-Value (KV) cache from FP16 models for all five inputs. 
While maintaining offline storage of prompts in real scenarios, this strategy negligibly impacts inference speed and significantly enhances model performance.
Notably, AWQ-PRONG achieves an average improvement of 0.98\% compared with AWQ across all model sizes. 
These findings affirm PRONG's simplicity and effectiveness in restoring the capabilities of quantized models.
Furthermore, in comparison to other state-of-the-art PTQ baselines like GPTQ and OmniQuant, AWQ-PRONG demonstrates superior performance in all Vicuna-v1.3 model sizes. 
For instance, the 13B model with AWQ-PRONG reports a remarkable accuracy gain of 2.38\% over the OmniQuant method.
This superiority is even more pronounced under five-shot settings, underscoring the efficacy of retaining full-precision prompts KV cache in improving the performance of quantized models, particularly in conversational scenarios.




\paragraph{Results on Commonsense QA tasks.}
We further evaluate the quantized Vicuna models on zero-shot commonsense QA tasks.
The results of Vicuna-v1.5-13B, as detailed in Table \ref{tab:qa}, indicate that the PivotKV enables notable improvements of the AWQ method, especially under low-bit quantization.
The final model surpasses the results of GPTQ and Omni
The average accuracy of other sizes of Vicuna models is presented in Table \ref{tab:all-models} and our AWQ-PivotKV yields the best zero-shot performance.
These superior results strongly demonstrate the efficacy of our improved PivotKV Cache.


% \lin{Need to rewrite.}
% In our continued evaluation, AWQ-PRONG is applied to zero-shot commonsense QA tasks under both INT4-g128 and INT3-g128 configurations. 
% The results, as detailed in Table \ref{tab:qa}, indicate that AWQ-PRONG marks a substantial enhancement over the AWQ quantized models and also exceeds the results of GPTQ and OmniQuant across all 7B and 13B models.
% Particularly noteworthy is the performance of AWQ-PRONG on INT3-g128 quantized models, where it surpasses the leading method OmniQuant by an average margin of 0.81.
% This edge indicates the potential for further improvements, especially with integrating more suitable prompts and our proposed \lin{prompt KV Cache} strategy.


% ================ Table MMLU
\begin{table*}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|ccccc|ccccc}
\toprule
% \multicolumn{1}{c|}{\multirow{2}{*}{Model}} & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{5}{c|}{MMLU (0 shot)}                                                                                & \multicolumn{5}{c}{MMLU (5 shot)}                                                                                \\ \cmidrule{3-12} 
% \multicolumn{1}{c|}{}                       & \multicolumn{1}{c|}{}                        & Hums                 & STEM                 & Social               & Others               & Avg.                  & Hums                 & STEM                 & Social               & Others               & Avg.                 \\ 
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}}    & \multicolumn{5}{c|}{\textbf{MMLU (0 shot)}}    & \multicolumn{5}{c}{\textbf{MMLU (5 shot)}}       \\ \cmidrule{3-12} 
\multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{}              & \textbf{Hums}        & \textbf{STEM}        & \textbf{Social}      & \textbf{Others}      & \textbf{Avg.}         & \textbf{Hums}        & \textbf{STEM}        & \textbf{Social}      & \textbf{Others}      & \textbf{Avg.}  \\
\midrule
\multirow{6}{*}{Vicuna-V1.3-7B}             & FP16                                         & 44.31\%              & 36.28\%              & 53.23\%              & 53.70\%              & 46.71\%               & 44.23\%              & 38.34\%              & 53.82\%              & 53.15\%              & 47.12\%              \\ \cmidrule{2-12} 
                                            & RTN                                          & 38.09\%              & 31.58\%              & 42.35\%              & 44.32\%              & 39.06\%               & 36.81\%              & 32.77\%              & 43.87\%              & 44.79\%              & 39.33\%              \\
                                            & GPTQ                                          & 39.06\%              & 32.50\%              & 44.52\%              & 46.85\%              & 40.65\%               & 36.92\%              & 33.96\%              & 45.11\%              & 45.81\%              & 40.13\%              \\
                                            & AWQ                                          & 40.49\%              & 32.44\%              & 47.06\%              & 49.57\%              & 42.29\%               & 39.64\%              & 36.22\%              & 48.72\%              & 49.11\%              & 43.08\%              \\
                                            & OmniQuant                                    & 41.36\%              & 33.96\%              & 47.42\%              & 47.69\%              & 42.56\%               & 41.15\%              & 35.45\%              & 48.20\%              & 48.58\%              & 43.18\%              \\
                                            & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias}                         & \textbf{42.38\%}     & \textbf{34.26\%}     & \textbf{48.33\%}     & \textbf{50.86\%}     & \textbf{43.90\%}      & \textbf{41.74\%}     & \textbf{36.85\%}     & \textbf{50.67\%}     & \textbf{50.93\%}     & \textbf{44.77\%}     \\ 
\midrule
\multirow{6}{*}{Vicuna-V1.3-13B}            & FP16                                         & 47.89\%              & 39.96\%              & 58.86\%              & 57.34\%              & 50.77\%               & 49.78\%              & 40.46\%              & 60.61\%              & 58.24\%              & 52.10\%              \\ \cmidrule{2-12} 
                                            & RTN                                          & 42.06\%              & 32.87\%              & 47.61\%              & 49.51\%              & 43.02\%                 & 42.42\%              & 34.46\%              & 50.34\%              & 51.57\%              & 44.56\%              \\
                                            & GPTQ                                           & 45.14\%              & 35.82\%              & 52.23\%              & 51.17\%              & 46.08\%                  & 45.74\%              & 37.51\%              & 54.89\%              & 53.70\%              & 47.81\%              \\
                                            & AWQ                                          & 45.14\%              & 36.18\%              & 52.55\%              & 53.79\%              & 46.84\%               & 46.65\%              & 37.64\%              & 55.54\%              & 54.87\%              & 48.56\%              \\
                                            & OmniQuant                                    & 43.29\%              & 36.65\%              & 51.64\%              & 53.05\%              & 45.95\%               & 45.29\%              & 37.84\%              & 55.02\%              & 54.38\%              & 47.92\%              \\
                                            & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias}                         & \textbf{46.72\%}     & \textbf{37.51\%}     & \textbf{54.11\%}     & \textbf{55.24\%}     & \textbf{48.33\%}      & \textbf{46.52\%}     & \textbf{38.10\%}     & \textbf{56.19\%}     & \textbf{55.52\%}     & \textbf{48.91\%}     \\ 
\midrule
\multirow{6}{*}{Vicuna-V1.3-33B}            & FP16                                         & 53.73\%              & 44.14\%              & 67.63\%              & 63.54\%              & 56.98\%               & 57.66\%              & 46.32\%              & 69.32\%              & 64.25\%              & 59.30\%              \\ \cmidrule{2-12} 
                                            & RTN                                          & 49.88\%              & 40.13\%              & 61.33\%              & 58.42\%              & 52.26\%               & 51.26\%              & 42.54\%              & 61.75\%              & 57.71\%              & 53.18\%              \\
                                            & GPTQ                                         & 51.18\%              & 40.06\%              & 61.81\%              & 59.50\%              & 53.04\%               & 54.05\%              & 44.07\%              & 64.38\%              & 61.32\%              & 55.85\%              \\
                                            & AWQ                                          & 51.69\%              & 42.74\%              & 63.41\%              & 61.38\%              & 54.57\%               & 54.56\%              & 44.10\%              & 65.36\%              & 60.67\%              & 56.09\%              \\
                                            & OmniQuant                                    & 51.14\%              & 42.08\%              & 63.60\%              & 59.84\%              & 53.93\%               & 53.77\%              & 43.80\%              & 63.47\%              & 59.69\%              & 55.12\%              \\
                                            & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias}                         & \textbf{52.20\%}     & \textbf{43.11\%}     & \textbf{63.93\%}     & \textbf{62.06\%}     & \textbf{55.09\%}      & \textbf{55.94\%}     & \textbf{43.97\%}              & \textbf{65.88\%}     & \textbf{61.60\%}     & \textbf{56.85\%}     \\ 
\midrule
\multirow{6}{*}{Vicuna-V1.5-7B}             & FP16                                         & 45.40\%              & 38.67\%              & 56.16\%              & 55.92\%              & 48.74\%               & 45.78\%              & 39.50\%              & 58.14\%              & 57.46\%              & 49.84\%              \\ \cmidrule{2-12} 
                                            & RTN                                          & 42.06\%              & 34.16\%              & 50.47\%              & 50.59\%              & 44.17\%               & 40.68\%              & 38.60\%              & 50.31\%              & 50.56\%              & 44.62\%              \\
                                            & GPTQ                                         & 39.81\%              & 32.97\%              & 48.29\%              & 48.49\%              & 42.20\%               & 40.32\%              & 36.25\%              & 50.76\%              & 50.00\%              & 43.97\%              \\
                                            & AWQ                                          & 42.08\%              & 35.55\%              & 51.61\%              & 51.54\%              & 44.95\%               & 42.55\%              & 38.93\%              & 53.10\%              & 52.78\%              & 46.45\%              \\
                                            & OmniQuant                                    & 42.57\%              & 35.98\%              & 51.64\%              & \textbf{53.55\%}     & \textbf{45.68\%}               & 42.95\%              & 37.57\%              & 53.59\%              & \textbf{53.39\% }             & 46.54\%              \\
                                            & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias}                        & \textbf{42.57\%}     & \textbf{36.15\%}     & \textbf{51.84\%}             & 51.70\%              & 45.33\%               & \textbf{43.32\%}     & \textbf{39.66\%}     & \textbf{54.08\%}     & 52.65\%              & \textbf{47.04\%}     \\ 
\midrule
\multirow{6}{*}{Vicuna-V1.5-13B}            & FP16                                         & 50.48\%              & 43.70\%              & 62.72\%              & 62.74\%              & 54.54\%               & 51.97\%              & 44.96\%              & 65.26\%              & 62.40\%              & 55.78\%              \\ \cmidrule{2-12} 
                                            & RTN                                          & 46.61\%              & 41.32\%              & 58.92\%              & 57.53\%              & 50.69\%               & 47.14\%              & 42.81\%              & 59.38\%              & 58.17\%              & 51.44\%              \\
                                            & GPTQ                                         & 48.27\%                    & 40.95\%          & 59.31\%          & 57.96\%              & 51.35\%                          & 49.56\%          & 43.01\%          & 60.25\%          & 60.02\%              & 52.91\%          \\
                                            & AWQ                                          & 48.82\%              & 41.72\%              & 61.03\%              & 58.30\%              & 52.16\%               & 49.52\%              & 43.01\%              & 61.72\%              & 58.73\%              & 52.92\%              \\
                                            & OmniQuant                                    & \textbf{49.52\%}              & 41.22\%              & 59.47\%              & 57.74\%              & 51.82\%               & 49.12\%              & \textbf{44.40\% }             & 60.48\%              & 58.95\%              & 52.86\%              \\
                                            & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias}                         & 49.33\%              & \textbf{42.28\%}     & \textbf{61.39\%}     & \textbf{59.13\%}     & \textbf{52.72\%}      & \textbf{50.82\%}     & 43.51\%              & \textbf{62.63\%}     & \textbf{60.58\%}     & \textbf{54.09\%}     \\ 
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{INT3-group128 quantization results on MMLU benchmarks
}
\vspace{-1em}
\label{tab:mmlu}
\end{table*}





% ===============


\begin{table*}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Vicuna-V1.5-13B}}        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{5}{c|}{\textbf{MMLU (0 shot)}}    & \multicolumn{5}{c}{\textbf{MMLU (5 shot)}} \\ \cmidrule{3-12} 
\multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{}       & \textbf{Hums}    & \textbf{STEM}    & \textbf{Social}  & \textbf{Others}  & \textbf{Avg.}    & \textbf{Hums}    & \textbf{STEM}    & \textbf{Social}  & \textbf{Others}  & \textbf{Avg.}    \\ 
\midrule
FP16      & -   & 50.48\%          & 43.70\%          & 62.72\%          & 62.74\%          & 54.54\%          & 51.97\%          & 44.96\%          & 65.26\%          & 62.40\%          & 55.78\%          \\ 
\midrule
\multirow{5}{*}{INT3-g128} 
& RTN           & 46.61\%          & 41.32\%          & 58.92\%          & 57.53\%          & 50.69\%          & 47.14\%          & 42.81\%          & 59.38\%          & 58.17\%          & 51.44\%          \\
& GPTQ          & 48.27\%          & 40.95\%          & 59.31\%          & 57.96\%          & 51.35\%          & 49.56\%          & 43.01\%          & 60.25\%          & 60.02\%          & 52.91\%          \\
& AWQ           & 48.82\%          & 41.72\%          & 61.03\%          & 58.30\%          & 52.16\%          & 49.52\%          & 43.01\%          & 61.72\%          & 58.73\%          & 52.92\%          \\
& OmniQuant     & \textbf{49.52\%} & 41.22\%          & 59.47\%          & 57.74\%          & 51.82\%          & 49.12\%          & \textbf{44.40\%} & 60.48\%          & 58.95\%          & 52.86\%          \\
& \rowcolor{orange!10} 
AWQ+BOS\_kv   & 49.31\%          & \textbf{42.18\%} & \textbf{61.20\%} & \textbf{59.28\%} & \textbf{52.68\%} & \textbf{50.31\%} & 43.37\%          & \textbf{61.91\%} & \textbf{59.93\%} & \textbf{53.58\%} \\ 
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{INT3-group128 quantization results on MMLU benchmarks
}
% \vspace{-1em}
\label{tab:mmlu}
\end{table*}








% ================
\begin{table*}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{5}{c|}{\textbf{MMLU (0 shot)}}    & \multicolumn{5}{c}{\textbf{MMLU (5 shot)}} \\ \cmidrule{3-12} 
\multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{}       & \textbf{Hums}    & \textbf{STEM}    & \textbf{Social}  & \textbf{Others}  & \textbf{Avg.}    & \textbf{Hums}    & \textbf{STEM}    & \textbf{Social}  & \textbf{Others}  & \textbf{Avg.}    \\ 
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Vicuna-V1.5-13B\\ INT3-g128\end{tabular}} 
& FP16          & 50.48\%          & 43.70\%          & 62.72\%          & 62.74\%          & 54.54\%          & 51.97\%          & 44.96\%          & 65.26\%          & 62.40\%          & 55.78\%          \\ 
& RTN           & 46.61\%          & 41.32\%          & 58.92\%          & 57.53\%          & 50.69\%          & 47.14\%          & 42.81\%          & 59.38\%          & 58.17\%          & 51.44\%          \\
& GPTQ          & 48.27\%          & 40.95\%          & 59.31\%          & 57.96\%          & 51.35\%          & 49.56\%          & 43.01\%          & 60.25\%          & 60.02\%          & 52.91\%          \\
& AWQ           & 48.82\%          & 41.72\%          & 61.03\%          & 58.30\%          & 52.16\%          & 49.52\%          & 43.01\%          & 61.72\%          & 58.73\%          & 52.92\%          \\
& OmniQuant     & \textbf{49.52\%} & 41.22\%          & 59.47\%          & 57.74\%          & 51.82\%          & 49.12\%          & \textbf{44.40\%} & 60.48\%          & 58.95\%          & 52.86\%          \\
& \rowcolor{orange!10} 
AWQ+BOS\_kv   & 49.31\%          & \textbf{42.18\%} & \textbf{61.20\%} & \textbf{59.28\%} & \textbf{52.68\%} & \textbf{50.31\%} & 43.37\%          & \textbf{61.91\%} & \textbf{59.93\%} & \textbf{53.58\%} \\ 
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{INT3-group128 quantization results on MMLU benchmarks
}
% \vspace{-1em}
\label{tab:mmlu}
\end{table*}


% ================


\begin{table*}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|l|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{5}{c|}{\textbf{MMLU (0 shot)}}    & \multicolumn{5}{c}{\textbf{MMLU (5 shot)}} \\ \cmidrule{3-12} 
\multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{}       & \textbf{Hums}    & \textbf{STEM}    & \textbf{Social}  & \textbf{Others}  & \textbf{Avg.}    & \textbf{Hums}    & \textbf{STEM}    & \textbf{Social}  & \textbf{Others}  & \textbf{Avg.}    \\ 
\midrule
FP16      & -   & 50.48\%          & 43.70\%          & 62.72\%          & 62.74\%          & 54.54\%          & 51.97\%          & 44.96\%          & 65.26\%          & 62.40\%          & 55.78\%          \\ 
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Vicuna-V1.5-13B\\ INT3-g128\end{tabular}} 
& RTN           & 46.61\%          & 41.32\%          & 58.92\%          & 57.53\%          & 50.69\%          & 47.14\%          & 42.81\%          & 59.38\%          & 58.17\%          & 51.44\%          \\
& GPTQ          & 48.27\%          & 40.95\%          & 59.31\%          & 57.96\%          & 51.35\%          & 49.56\%          & 43.01\%          & 60.25\%          & 60.02\%          & 52.91\%          \\
& AWQ           & 48.82\%          & 41.72\%          & 61.03\%          & 58.30\%          & 52.16\%          & 49.52\%          & 43.01\%          & 61.72\%          & 58.73\%          & 52.92\%          \\
& OmniQuant     & \textbf{49.52\%} & 41.22\%          & 59.47\%          & 57.74\%          & 51.82\%          & 49.12\%          & \textbf{44.40\%} & 60.48\%          & 58.95\%          & 52.86\%          \\
& \rowcolor{orange!10} 
AWQ+BOS\_kv   & 49.31\%          & \textbf{42.18\%} & \textbf{61.20\%} & \textbf{59.28\%} & \textbf{52.68\%} & \textbf{50.31\%} & 43.37\%          & \textbf{61.91\%} & \textbf{59.93\%} & \textbf{53.58\%} \\ 
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{INT3-group128 quantization results on MMLU benchmarks
}
% \vspace{-1em}
\label{tab:mmlu}
\end{table*}





% ================= Table Vicuna other models
\begin{table*}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|cccc|cccc}
\toprule
% \multirow{2}{*}{\textbf{\#bits}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{MMLU (5 shot)  average}}    & \multicolumn{4}{c}{\textbf{Common Sense QA (0   shot)  average}}            \\ \cmidrule{3-10} 
%                                  &                  & \textbf{v1.5-7B} & \textbf{v1.3-7B} & \textbf{v1.3-13B} & \textbf{v1.3-30B} & \textbf{v1.5-7B} & \textbf{v1.3-7B} & \textbf{v1.3-13B} & \textbf{v1.3-30B} \\ \midrule
\multicolumn{2}{c|}{\textbf{Task Acc}}            & \multicolumn{4}{c|}{\textbf{MMLU (5 shot)  average}}                        & \multicolumn{4}{c}{\textbf{Common Sense QA (0   shot)  average}}            \\ \cmidrule{3-10} 
\multicolumn{2}{c|}{\textbf{Vicuna v1.3 \& v1.5}} & \textbf{v1.5-7B} & \textbf{v1.3-7B} & \textbf{v1.3-13B} & \textbf{v1.3-30B} & \textbf{v1.5-7B} & \textbf{v1.3-7B} & \textbf{v1.3-13B} & \textbf{v1.3-30B} \\ \midrule
FP16                             & -                & 49.84\%          & 47.12\%          & 52.10\%          & 59.30\%          & 52.09\%          & 52.09\%          & 52.09\%          & 52.84\%          \\ \midrule
\multirow{5}{*}{w3a16g128}       & RTN              & 44.62\%          & 39.33\%          & 44.56\%          & 53.18\%          & 45.42\%          & 45.42\%          & 45.42\%          & 45.69\%          \\
                                 & GPTQ             & 43.99\%          & 40.12\%          & 47.83\%          & 55.84\%          & 46.95\%          & 46.95\%          & 46.95\%          & 47.93\%          \\
                                 & AWQ              & 46.45\%          & 43.08\%          & 48.56\%          & 56.09\%          & 48.55\%          & 48.55\%          & 48.55\%          & 49.24\%          \\
                                 & Omniquant        & 46.54\%          & 43.18\%          & 47.92\%          & 55.12\%          & 48.19\%          & 48.19\%          & 48.19\%          & 48.74\%          \\
                                 & \rowcolor{orange!10}
                                 AWQ+BOS\_kv      & \textbf{46.87\%} & \textbf{44.67\%} & \textbf{49.05\%} & \textbf{56.91\%} & \textbf{49.38\%} & \textbf{49.38\%} & \textbf{49.38\%} & \textbf{50.21\%} \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{INT3-goup128 quantization results on various Vicuna models
}
% \vspace{-1em}
\label{tab:qa}
\end{table*}



% ================ Table QA
\begin{table*}[!t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l|lccccclcc}
\toprule
% Model       & \#bits                      & Method           & OBQA                                    & WinoGrande       & ARC-C            & ARC-E            & PIQA             & BoolQ                                & HellaSwag        & Avg              \\ 
\textbf{Model}    & \textbf{\#bits}    & \textbf{Method}     & \textbf{OBQA}                        & \textbf{WinoGrande} & \textbf{ARC-C}  & \textbf{ARC-E}   & \textbf{PIQA}    & \textbf{BoolQ}                    & \textbf{HellaSwag} & \textbf{Avg.}\\ 
\midrule
            & FP16                        & -                & 43.80\%                                 & 69.46\%          & 44.54\%          & 71.89\%          & 79.16\%          & 78.07\%                              & 73.93\%          & 65.84\%          \\ \cmidrule{2-11} 
            &                             & RTN              & 41.00\%                                 & 64.64\%          & 39.08\%          & 65.03\%          & 74.92\%          & 75.81\%                              & 68.59\%          & 61.30\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 41.60\%                                 & 67.96\%          & 38.65\%          & 65.95\%          & 76.44\%          & 76.36\%                              & 71.27\%          & 62.60\%          \\
            &                             & OmniQuant        & 42.00\%                                 & 67.88\%          & 40.02\%          & 66.75\%          & 75.84\%          & 75.41\%                              & 70.52\%          & 62.63\%          \\
            & \multirow{-5}{*}{w3a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias}    & \textbf{43.40\%}   & \textbf{67.72\%} & \textbf{39.33\%} & \textbf{68.01\%} & \textbf{77.26\%} & \textbf{78.75\%}       & 70.78\%       & \textbf{63.61\%}      \\ \cmidrule{2-11} 
            &                             & RTN              & 41.80\%                                 & 67.80\%          & 44.45\%          & 69.91\%          & 77.86\%          & 75.57\%                              & 73.25\%          & 64.38\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 42.80\%                                 & 67.09\%          & 43.43\%          & 71.34\%          & 77.91\%          & 76.36\%                              & 73.46\%          & 64.63\%          \\
            &                             & OmniQuant        & 42.40\%                                 & 68.98\%          & 44.03\%          & 71.04\%          & 78.29\%          & 76.97\%                              & 73.19\%          & 64.99\%          \\
\multirow{-11}{*}{Vicuna-V1.3-7B}  
            & \multirow{-5}{*}{w4a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & \textbf{43.60\%}  & \textbf{68.35\%} & \textbf{43.34\%} & \textbf{71.80\%} & \textbf{78.24\%} & \multicolumn{1}{c}{\textbf{77.06\%}} & \textbf{73.37\%} & \textbf{65.11\%} \\ 
\midrule
            & FP16                        & -                & 45.40\%                                 & 71.03\%          & 47.70\%          & 73.70\%          & 78.84\%          & 82.81\%                              & 77.00\%          & 68.07\%          \\ \cmidrule{2-11} 
            &                             & RTN              & 42.20\%                                 & 69.77\%          & 44.03\%          & 68.14\%          & 76.71\%          & 80.52\%                              & 73.28\%          & 64.95\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 42.60\%                                 & 68.75\%          & 45.90\%          & 69.57\%          & 77.75\%          & 80.80\%                              & 74.78\%          & 65.74\%          \\
            &                             & OmniQuant        & 43.60\%                                 & 70.56\%          & 44.62\%          & 70.66\%          & 77.15\%          & 81.28\%                              & 74.13\%          & 66.00\%          \\
            & \multirow{-5}{*}{w3a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & 43.20\%           & 69.06\%          & \textbf{45.99\%} & \textbf{70.96\%} & \textbf{77.91\%} & \textbf{81.53\%}                     & \textbf{75.06\%} & \textbf{66.24\%} \\ 
            \cmidrule{2-11} 
            &                             & RTN              & 43.80\%                                 & 71.19\%          & 47.01\%          & 72.64\%          & 78.18\%          & 82.35\%                              & 76.19\%          & 67.34\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 44.00\%                                 & 70.01\%          & 46.67\%          & 72.64\%          & 78.62\%          & 82.66\%                              & 76.43\%          & 67.29\%          \\
            &                             & OmniQuant        & 45.80\%                                 & 71.35\%          & 46.08\%          & 72.14\%          & 78.73\%          & 82.35\%                              & 76.34\%          & 67.54\%          \\
\multirow{-11}{*}{Vicuna-V1.3-13B} 
            & \multirow{-5}{*}{w4a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & 45.60\%           & \textbf{71.11\%} & \textbf{47.35\%} & \textbf{73.40\%} & \textbf{78.24\%} & \textbf{82.78\%}                     & \textbf{76.80\%} & \textbf{67.90\%} \\ 
\midrule
            & FP16                        & -                & 45.40\%                                 & 71.03\%          & 47.70\%          & 73.70\%          & 78.84\%          & 82.81\%                              & 77.00\%          & 68.07\%          \\ \cmidrule{2-11} 
            &                             & RTN              & 46.00\%                                 & 72.45\%          & 49.83\%          & 71.63\%          & 78.73\%          & \multicolumn{1}{c}{82.75\%}          & 77.86\%          & 68.46\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 45.40\%                                 & 72.77\%          & 50.77\%          & 72.56\%          & 78.07\%          & \multicolumn{1}{c}{82.42\%}          & 78.33\%          & 68.62\%          \\
            &                             & OmniQuant        & 45.60\%                                 & 73.32\%          & 47.95\%          & 72.52\%          & 78.56\%          & \multicolumn{1}{c}{83.58\%}          & 78.05\%          & 68.51\%          \\
            & \multirow{-5}{*}{w3a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & \textbf{45.00\%}   & \textbf{73.56\%} & \textbf{51.71\%} & \textbf{72.81\%} & \textbf{78.62\%} & \multicolumn{1}{c}{82.54\%}          & \textbf{78.61\%} & \textbf{68.98\%} \\ 
            \cmidrule{2-11} 
            &                             & RTN              & 46.60\%                                 & 73.95\%          & 51.96\%          & 74.07\%          & 78.84\%          & 83.43\%                              & 80.01\%          & 69.84\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 46.20\%                                 & 73.40\%          & 50.60\%          & 73.53\%          & 79.76\%          & \multicolumn{1}{c}{84.04\%}          & 79.91\%          & 69.63\%          \\
            &                             & OmniQuant        & 47.60\%                                 & 73.72\%          & 51.96\%          & 73.32\%          & 79.38\%          & \multicolumn{1}{c}{83.58\%}          & 79.85\%          & \textbf{69.92\%} \\
\multirow{-11}{*}{Vicuna-V1.3-33B} 
            & \multirow{-5}{*}{w4a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & 46.00\%                                 & \textbf{73.56\%} & 50.60\%          & \textbf{74.16\%} & 79.60\%          & \multicolumn{1}{c}{\textbf{84.22\%}} & 79.70\%          & 69.69\%          \\ 
\midrule
            & FP16                        & -                & 45.00\%                                 & 69.53\%          & 45.73\%          & 71.25\%          & 78.02\%          & 80.92\%                              & 73.78\%          & 66.32\%          \\ \cmidrule{2-11} 
            &                             & RTN              & 39.40\%                                 & 66.22\%          & 43.34\%          & 67.72\%          & 76.12\%          & 77.40\%                              & 71.71\%          & 63.13\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 40.80\%                                 & 67.01\%          & 43.34\%          & 67.55\%          & 75.14\%          & 78.32\%                              & 71.03\%          & 63.31\%          \\
            &                             & OmniQuant        & 41.40\%                                 & 66.22\%          & 43.52\%          & 67.26\%          & 76.33\%          & 77.13\%                              & 70.35\%          & 63.17\%          \\
            & \multirow{-5}{*}{w3a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & \textbf{41.60\%}    & \textbf{67.56\%} & 42.49\%          & \textbf{68.22\%} & 75.46\%          & \textbf{79.33\%}                     & 70.85\%          & \textbf{63.64\%} \\ 
            \cmidrule{2-11} 
            &                             & RTN              & 43.80\%                                 & 68.82\%          & 45.39\%          & 70.33\%          & 77.26\%          & 81.10\%                              & 73.31\%          & 65.72\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 43.40\%                                 & 68.75\%          & 45.39\%          & 70.66\%          & 77.20\%          & 81.35\%                              & 73.43\%          & 65.74\%          \\
            &                             & OmniQuant        & 43.00\%                                 & 68.75\%          & 44.28\%          & 70.50\%          & 76.71\%          & 81.01\%                              & 72.82\%          & 65.30\%          \\
\multirow{-11}{*}{Vicuna-V1.5-7B}  
            & \multirow{-5}{*}{w4a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & \textbf{44.00\%}   & \textbf{69.06\%} & \textbf{45.65\%} & \textbf{71.63\%} & \textbf{77.86\%} & \textbf{82.35\%}                     & 73.39\%          & \textbf{66.28\%} \\ 
\midrule
            & FP16                        & -                & 45.40\%                                 & 71.51\%          & 50.68\%          & 74.87\%          & 79.11\%          & 85.29\%                              & 77.50\%          & 69.19\%          \\ \cmidrule{2-11} 
            &                             & RTN              & 42.00\%                                 & 70.01\%          & 47.44\%          & 72.77\%          & 77.58\%          & 82.20\%                              & 74.18\%          & 66.60\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 44.00\%                                 & 68.75\%          & 48.21\%          & 71.76\%          & 78.18\%          & 83.58\%                              & 75.09\%          & 67.08\%          \\
            &                             & OmniQuant        & 43.40\%                                 & 68.51\%          & 47.53\%          & 71.09\%          & 77.53\%          & 82.32\%                              & 73.92\%          & 66.33\%          \\
            & \multirow{-5}{*}{w3a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & \textbf{45.80\%}    & \textbf{70.64\%} & \textbf{48.63\%} & \textbf{72.35\%} & 76.99\%          & 85.23\%                              & \textbf{75.21\%} & \textbf{67.84\%} \\ 
            \cmidrule{2-11} 
            &                             & RTN              & 44.20\%                                 & 70.80\%          & 48.98\%          & 73.82\%          & 78.73\%          & 84.68\%                              & 76.36\%          & 68.22\%          \\
            &                             & GPTQ             &                                         &                  &                  &                  &                  &                                      &                  &                  \\
            &                             & AWQ              & 44.00\%                                 & 72.06\%          & 49.15\%          & 73.44\%          & 78.78\%          & 85.17\%                              & 77.00\%          & 68.51\%          \\
            &                             & OmniQuant        & 43.80\%                                 & 70.24\%          & 49.74\%          & 73.61\%          & 78.78\%          & 84.59\%                              & 76.35\%          & 68.16\%          \\
\multirow{-11}{*}{Vicuna-V1.5-13B} 
            & \multirow{-5}{*}{w4a16g128} & \rowcolor{orange!10} \textbf{AWQ+prompt+gbias} & \textbf{45.80\%}   & \textbf{72.85\%} & \textbf{49.74\%} & \textbf{74.28\%} & 78.73\%          & \textbf{85.66\%}                     & \textbf{77.25\%} & \textbf{69.19\%} \\ 
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-10pt}
\caption{QA tasks
}
\vspace{-1em}
\label{tab:qa}
\end{table*}
